Positivity results for Stanley's character polynomials

Stanley introduced expressions for the normalized characters of the symmetric group and stated some positivity conjectures for these expressions. Here, we give an affirmative partial answer to Stanley's positivity conjectures about the expressions using results on Kerov polynomials. In particular, we use new positivity results by Goulden and the present author. We shall see that the generating series $C(t)$ introduced by them is critical to our discussion.

==> thmstuff.tex <==
%theorems, lemmas and things like that

\theoremstyle{plain}
\RequirePackage{latexsym}
%\theoremsymbol{\ensuremath{\Box}}
\theoremseparator{.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% basic theorem environments

\newtheorem{theorem}{Theorem}[section]
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{notation}{Notation}
\newtheorem{defn}{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{proposition}[theorem]{Proposition}

{\theorembodyfont{\normalfont} \theoremsymbol{\ensuremath{\Box}}
\newtheorem{example}[theorem]{Example}}
{\theorembodyfont{\normalfont} \theoremsymbol{\ensuremath{\Box}}
\newtheorem{remark}{Remark}}
{\theorembodyfont{\normalfont} \newtheorem{quest}{Question}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%proof environment

\theoremstyle{nonumberplain}
\theoremheaderfont{\it}
\theorembodyfont{\normalfont}
\RequirePackage{latexsym}
\theoremsymbol{\ensuremath{\Box}}
\RequirePackage{amssymb}
\newtheorem{proof}{Proof}

%proof of environment

\theoremstyle{empty}
\theoremheaderfont{\bf}
\theorembodyfont{\normalfont}
\RequirePackage{latexsym}
\theoremsymbol{\ensuremath{\Box}}
\RequirePackage{amssymb}
\newtheorem{proofof}{Proof}


%margin size
\setlength{\hoffset}{-1in}              %`driver' margin
\setlength{\voffset}{-0.75in}           %`driver' margin
\setlength{\textwidth}{5.5in}           %width of text body
\setlength{\textheight}{8.5in}            %height of text body
\setlength{\evensidemargin}{1.5in}        %driver margin to body
\setlength{\oddsidemargin}{1.5in}         %driver margin to body
%\setlength{\topmargin}{0in}             %from driver margin to header
%\setlength{\marginparwidth}{0pt}
%\setlength{\marginparsep}{0pt}         %horizontal space between
%\setlength{\marginparpush}{0pt}        %min space between par
%\setlength{\headsep}{0pt}
%\setlength{\headheight}{0pt}
\setlength{\footskip}{0.5in}
%\setlength{\linewidth}{0pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%solution environment

\theoremstyle{nonumberplain}
\theoremheaderfont{\it}
\theorembodyfont{\normalfont}
\RequirePackage{latexsym}
\theoremsymbol{\ensuremath{\Box}}
\RequirePackage{amssymb}
\newtheorem{sol}{Solution}

%margin size
\setlength{\hoffset}{-1in}              %`driver' margin
\setlength{\voffset}{-0.75in}           %`driver' margin
\setlength{\textwidth}{5.5in}           %width of text body
\setlength{\textheight}{8.5in}            %height of text body
\setlength{\evensidemargin}{1.5in}        %driver margin to body
\setlength{\oddsidemargin}{1.5in}         %driver margin to body
%\setlength{\topmargin}{0in}             %from driver margin to header
%\setlength{\marginparwidth}{0pt}
%\setlength{\marginparsep}{0pt}         %horizontal space between
%\setlength{\marginparpush}{0pt}        %min space between par
%\setlength{\headsep}{0pt}
%\setlength{\headheight}{0pt}
\setlength{\footskip}{0.5in}
%\setlength{\linewidth}{0pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: "thmstuff"
%%% End: 

